Developing a Recommendation Benchmark for MLPerf Training and Inference

Deep learning-based recommendation models are used pervasively and broadly, for example, to recommend movies, products, or other information most relevant to users, in order to enhance the user experience. Among various application domains which have received significant industry and academia research attention, such as image classification, object detection, language and speech translation, the performance of deep learning-based recommendation models is less well explored, even though recommendation tasks unarguably represent significant AI inference cycles at large-scale datacenter fleets. To advance the state of understanding and enable machine learning system development and optimization for the commerce domain, we aim to define an industry-relevant recommendation benchmark for the MLPerf Training andInference Suites. The paper synthesizes the desirable modeling strategies for personalized recommendation systems. We lay out desirable characteristics of recommendation model architectures and data sets. We then summarize the discussions and advice from the MLPerf Recommendation Advisory Board.

==> table/frameworks.tex <==
\begin{table}[t]
 \caption{Summary of software framework versus hardware architecture in the closed division. The hardware benchmarking involves many different frameworks. Preventing submitters from reimplementing the benchmark would have made it impossible to support the diversity of systems tested.}
 \label{tab:frameworks}
 \vskip 0.05in
  \begin{center}
 \begin{sc}
\begin{adjustbox}{width=\columnwidth, center}
\fontsize{4.3}{5.0}
\selectfont
\begin{tabular}{c | c | c | c | c | c }
\toprule
 & \textbf{ASIC} & \textbf{CPU} & \textbf{DSP}  & \textbf{FPGA} & \textbf{GPU} \\
\midrule
\textbf{Arm NN} &  & X &  &  & X \\
\hline
\textbf{Furiosa-AI} & & & & X & \\
\hline
\textbf{Hailo SDK} & X & & & &  \\
\hline
\textbf{HanGuang-AI} & X & & & &  \\
\hline
\textbf{ONNX} &  & X & & & \\
\hline
\textbf{OpenVino} &  & X & & & \\
\hline
\textbf{PyTorch} &  & X & & & \\
\hline
\textbf{SNPE} & & & X & &  \\
\hline
\textbf{Synapse} & X &  & & &  \\
\hline
\textbf{TensorFlow} & X & X & & & X \\
\hline
\textbf{TF-Lite} & & X & & & \\
\hline
\textbf{TensorRT} & & & & & X \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{center}
\vskip -0.15in
\end{table}

==> table/latency_constraints.tex <==
\begin{table}[h!] 
 \caption{Latency constraints for each task in the multistream and server scenarios.}
 \label{tab:latency}
 \vskip 0.05in
  \begin{center}
 \begin{small}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c  }
\toprule
\textbf{Task} & \begin{tabular}[c]{@{}c@{}}\textbf{Multistream}\\ \textbf{Arrival Time}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Server QoS}\\ \textbf{Constraint}\end{tabular}\\
\midrule
Image classification (heavy) & ~~50 ms & ~~15 ms \\
\hline
Image classification (light) & ~~50 ms & ~~10 ms \\
\hline
Object detection (heavy) & ~~66 ms & 100 ms \\
\hline
Object detection (light) & ~~50 ms & ~~10 ms \\
\hline
Machine translation & 100 ms & 250 ms \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

==> table/ml_task.tex <==
\begin{table*}[t] 
 \caption{ML Tasks in MLPerf Inference v0.5. Each one reflects critical commercial and research use cases for a large class of submitters, and together they also capture a broad set of computing motifs (e.g., CNNs and RNNs).}
 \label{tab:ml_task}
  \vskip 0.05in
  \begin{center}
 \begin{small}
 \begin{sc}
 \begin{adjustbox}{width=\textwidth, center}
\begin{tabular}{c | c | c |c | c }
\toprule
\textbf{Area} & \textbf{Task} & \textbf{Reference Model} & \textbf{Data Set} & \textbf{Quality Target} \\
\midrule
Vision & Image classification (heavy) & \begin{tabular}[c]{@{}c@{}}ResNet-50 v1.5\\ ~25.6M parameters\\ 7.8 GOPS / input\end{tabular}
& ImageNet (224x224)
& 99\% of FP32 (76.456\%) Top-1 accuracy \\
\hline
Vision & Image classification (light) & \begin{tabular}[c]{@{}c@{}}MobileNet-v1 224\\ ~4.2M parameters\\ 1.138 GOPS / input\end{tabular}
& ImageNet (224x224)
& 98\% of FP32 (71.676\%) Top-1 accuracy \\
\hline
Vision & Object detection (heavy) & \begin{tabular}[c]{@{}c@{}}SSD-ResNet34\\ 36.3M parameters\\ 433 GOPS / input\end{tabular}
& COCO (1,200x1,200)
& 99\% of FP32 (0.20 mAP) \\
\hline
Vision & Object detection (light) & \begin{tabular}[c]{@{}c@{}}SSD-MobileNet-v1\\ 6.91M parameters \\ 2.47 GOPS / input \end{tabular}
& COCO (300x300) 
& 99\% of FP32 (0.22 mAP) \\
\hline
Language & Machine translation & \begin{tabular}[c]{@{}c@{}}GNMT\\ ~210M parameters \end{tabular}
& WMT16 EN-DE
& 99\% of FP32 (23.9 SacreBleu)\\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table*}

==> table/model_queries.tex <==
\begin{table}[t] 
 \caption{Number of queries and samples per query for each task.}
 \label{tab:task_queries}
   \vskip 0.05in
  \begin{center}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c | c | c}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Number of Queries / Samples per Query}}   \\ \cline{2-5} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{\textbf{Single-stream}} & \multicolumn{1}{l|}{\textbf{Multistream}} & \multicolumn{1}{l|}{\textbf{Server}} & \multicolumn{1}{l}{\textbf{Offline}} \\ 
\midrule
Image classification (heavy) & 1K / 1 & 270K / $N$ & 270K / 1 & 1 / 24K \\
\hline
Image classification (light) & 1K / 1 & 270K / $N$ & 270K / 1 & 1 / 24K \\
\hline
Object detection (heavy) & 1K / 1 & 270K / $N$ & 270K / 1 & 1 / 24K \\
\hline
Object detection (light) & 1K / 1 & 270K / $N$ & 270K / 1 & 1 / 24K \\
\hline
Machine translation & 1K / 1 & 90K / $N$ & 90K / 1 & 1 / 24K \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{center}
\vskip -0.15in
\end{table}

==> table/performance_summary.tex <==
\begin{table}[b!] 
 \caption{Closed-division performance summary across tasks and scenarios. Each entry is the ratio of the highest to lowest performance. The performance range is as much as 10,000x. GNMT appears as N/A for multistream because it had no submissions.}
 \label{tab:performance}
    \vskip 0.05in
 \vskip 0.05in
  \begin{center}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c | c | c }
\toprule
 & \textbf{Single-Stream} & \textbf{Multistream} & \textbf{Server}  & \textbf{Offline} \\
\midrule
\textbf{GNMT} & 2 & N/A & 5 & 2,367 \\
\hline
\textbf{MobileNet-v1} & 1,199 & 29 & 9 & 438  \\
\hline
\textbf{ResNet-50v1.5} & 11154 & 27 & 26 & 10,289  \\
\hline
\textbf{SSD-MobileNet-v1} & 8 & 36 & 25 & 657 \\
\hline
\textbf{SSD-ResNet34} & 8 & 44 & 9 & 147 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{center}
\vskip -0.15in
\end{table}

==> table/query_requirements.tex <==
\begin{table}[t] 
 \caption{Query requirements for statistical confidence. All results must meet the minimum LoadGen scenario requirements.}
 \label{tab:statsconf}
    \vskip 0.05in
  \begin{center}
 \begin{small}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c | c | c}
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{Tail-Latency}\\ \textbf{Percentile}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Confidence}\\ \textbf{Interval}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Error}\\ \textbf{Margin}\end{tabular} & \textbf{Inferences} & \begin{tabular}[c]{@{}c@{}}\textbf{Rounded}\\ \textbf{Inferences}\end{tabular}\\
\midrule
90\% & 99\% & 0.50\% & 23,886 & $3\times2^{13} = 24,576$ \\
\hline
95\% & 99\% & 0.25\% & 50,425 & $7\times2^{13} = 57,344$\\
\hline
99\% & 99\% & 0.05\% & 262,742 & $33\times2^{13} = 270,336$ \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

==> table/scenarios_description.tex <==
\begin{table*}[t] 
 \caption{Scenario description and metrics. Each scenario targets a real-world use case based on customer and vendor input.}
 \label{tab:scenarios}
 \vskip 0.05in
  \begin{center}
 \begin{sc}
 \begin{adjustbox}{width=\textwidth, center}
\begin{tabular}{c | c | c |c | c }
\toprule
\textbf{Scenario} & \textbf{Query Generation} & \textbf{Metric} & \textbf{Samples/Query} & \textbf{Examples} \\
\midrule
Single-stream (SS) & Sequential
& 90th-percentile latency
& 1 & \begin{tabular}[c]{@{}c@{}}Typing autocomplete,\\ real-time AR\end{tabular}  \\
\hline
Multistream (MS) & Arrival interval with dropping
& \begin{tabular}[c]{@{}c@{}}Number of streams\\ subject to latency bound\end{tabular} 
& $N$ & \begin{tabular}[c]{@{}c@{}}Multicamera driver assistance,\\ large-scale automation\end{tabular}\\
\hline
Server (S) & Poisson distribution
& \begin{tabular}[c]{@{}c@{}}Queries per second\\ subject to latency bound\end{tabular} 
& 1 & Translation website \\
\hline
Offline (O) & Batch
& Throughput 
& At least 24,576 & Photo categorization \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{center}
\vskip -0.15in
\end{table*}

==> table/submissions.tex <==
\begin{table}[b!] 
 \caption{Closed-division submissions for the tasks and LoadGen scenarios. The high coverage of models and scenarios implies that the benchmark captures important real-world use cases.}
 \label{tab:submissions}
 \vskip 0.05in
  \begin{center}
 \begin{small}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c |c | c }
\toprule
 & \textbf{Single-Stream} & \textbf{Multistream} & \textbf{Server} & \textbf{Offline} \\
\midrule
\textbf{GNMT} & 2 & 0 & 6 & 11  \\
\hline
\textbf{MobileNet-v1} & 18 & 3 & 5 & 11  \\
\hline
\textbf{ResNet-50 v1.5} & 19 & 5 & 10 & 20 \\
\hline
\textbf{SSD-MobileNet-v1} & 8 & 3 & 5 & 13 \\
\hline
\textbf{SSD-ResNet34} & 4 & 4 & 7 & 12 \\
\hline\hline
\textbf{Total} & \textbf{51} & \textbf{15} & \textbf{33} & \textbf{67} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table}

==> tex/abstract.tex <==
Machine-learning (ML) hardware and software system demand is burgeoning. Driven by ML applications, the number of different ML inference systems has exploded. Over 100 organizations are building ML inference chips, and the systems that incorporate existing models span at least three orders of magnitude in power consumption and four orders of magnitude in performance; they range from embedded devices to data-center solutions. Fueling the hardware are a dozen or more software frameworks and libraries. The myriad combinations of ML hardware and ML software make assessing ML-system performance in an architecture-neutral, representative, and reproducible manner challenging. There is a clear need for industry-wide standard ML benchmarking and evaluation criteria. MLPerf Inference answers that call. Driven by more than 30 organizations as well as more than 200 ML engineers and practitioners, MLPerf implements a set of rules and practices to ensure comparability across systems with wildly differing architectures. In this paper, we present the method and design principles of the initial MLPerf Inference release. The first call for submissions garnered more than 600 inference-performance measurements from 14 organizations, representing over 30 systems that show a range of capabilities.

==> tex/benchmarks.tex <==
\section{Design and Implementation}
\label{sec:benchmarks}

In this section we describe the design and implementation of MLPerf Inference v0.5. We also define the components of an inference system (Section~\ref{sec:benchmarks:system}) and detail how an inference query flows through one such system (Section~\ref{sec:benchmarks:query_life}). Our discussion also covers the MLPerf Inference tasks for v0.5 (Section~\ref{sec:benchmarks:tasks}).

\subsection{Inference System Under Test (SUT)}
\label{sec:benchmarks:system}

A complete MLPerf Inference system contains multiple components: a data set, a system under test (SUT), the Load Generator (LoadGen), and an accuracy script. Figure~\ref{fig:SUT} shows an overview of an MLPerf Inference system. The data set, LoadGen, and accuracy script are fixed for all submissions and are provided by MLPerf. Submitters have wide discretion to implement an SUT according to their architecture's requirements and their engineering judgment. By establishing a clear boundary between submitter-owned and MLPerf-owned components, the benchmark maintains comparability among submissions.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.69\linewidth]{figures/Alternate_System_Under_Test.pdf}
    \caption{MLPerf Inference system under test (SUT) and how the components integrate. (1) The LoadGen requests that the SUT load samples; (2--3) the SUT loads samples into memory; (4) the SUT signals the LoadGen when it is ready; (5) the LoadGen issues requests to the SUT; (6) the benchmark processes the results and returns the results to the LoadGen; and (6) the LoadGen outputs logs, which the accuracy script then reads and verifies.}
    \label{fig:SUT}
    \vskip -0.15in
\end{figure}

\subsection{Life of a Query}
\label{sec:benchmarks:query_life}

At startup, the LoadGen requests that the SUT load samples into memory. The MLPerf Inference rules allow them to be loaded into DRAM as an untimed operation. The SUT loads the samples into DRAM and may perform other timed operations as the rules stipulate. These untimed operations may include but are not limited to compilation, cache warmup, and preprocessing. 

The SUT signals the LoadGen when it is ready to receive the first query. A query is a request for inference on one or more samples. The LoadGen sends queries to the SUT in accordance with the selected scenario. Depending on that scenario, it can submit queries one at a time, at regular intervals, or in a Poisson distribution. 

The SUT runs inference on each query and sends the response back to the LoadGen, which either logs the response or discards it. After the run, an accuracy script checks the logged responses to determine whether the model accuracy is within tolerance.

We provide a clear interface between the SUT and LoadGen so new scenarios and experiments can be handled in the LoadGen and rolled out to all models and SUTs without extra effort. Doing so also facilitates compliance and auditing, since many technical rules about query arrivals, timing, and accuracy are implemented outside of submitter code. As we describe in Section~\ref{sec:results_open_division}, one
submitter obtained results for over 60 image-classification and
object-detection models.

% As we describe in Section~\ref{sec:results_open_division}, one submitter benchmarked results for over a dozen image-classification and object-detection models.

Moreover, placing the performance-measurement code outside of submitter code is congruent with MLPerf's goal of end-to-end system benchmarking. To that end, the LoadGen measures the holistic performance of the entire SUT rather than any individual part. Finally, this condition enhances the benchmark's realism: inference engines typically serve as black-box components of larger systems.

\subsection{Benchmark Tasks}
\label{sec:benchmarks:tasks}

\input{table/ml_task.tex}

Designing ML benchmarks is fundamentally different from designing non-ML benchmarks. MLPerf defines high-level tasks (e.g., image classification) that a machine-learning system can perform. For each one, we provide a canonical reference model in a few widely used frameworks. The reference model and weights offer concrete instantiations of the ML task, but formal mathematical equivalence is unnecessary. For example, a fully connected layer can be implemented with different cache-blocking and evaluation strategies. Consequently, submitting results requires optimizations to achieve good performance. 

The concept of a reference model and a valid class of equivalent implementations creates freedom for most ML systems while still enabling relevant comparisons of inference systems. MLPerf provides reference models using 32-bit floating-point weights and, for convenience, also provides carefully implemented equivalent models to address the three most popular formats: TensorFlow~\cite{abadi2016tensorflow}, PyTorch~\cite{paszke2017pytorch}, and ONNX~\cite{bai2019onnx}.

% For the initial v0.5 of MLPerf Inference, we chose tasks that reflect key commercial and research usecases for a large class of submitters and also capture a broad set of computing motifs. In order to focus on the realistic rules and testing infrastructure, we opted for a minimum-viable-benchmark approach to accelerate the inference v0.5 development process. In future revisions of the benchmark, we plan to extend the scope to include more areas, tasks, models etc.

As Table~\ref{tab:ml_task} illustrates, we selected a set of vision and language tasks along with associated reference models. We chose vision and translation because they are widely used across all computing systems, from edge devices to cloud data centers. Additionally, mature and well-behaved reference models with different architectures (e.g., CNNs and RNNs) were available.

% Our decisions were made via a consensus-driven process and relied upon feedback from the  community to capture relevance in the selected models and data sets. Additionally, we aimed to maintain consistency and alignment between the training and inference benchmarks. Where possible we adopted models that were part of the training v0.6 suite, thereby amortizing the benchmark development effort. 

For the vision tasks, we defined both heavyweight and lightweight models. The former are representative of systems with greater compute resources, such as a data center or autonomous vehicle, where increasing the computation cost for better accuracy is a reasonable trade-off. In contrast, the latter models are appropriate for systems with constrained compute resources and low latency requirements, such as smartphones and low-cost embedded devices. 

For all tasks, we standardized on free and publicly available data sets to ensure the entire community can participate. Because of licensing restrictions on some data sets (e.g., ImageNet), we do not host them directly. Instead, the data is downloaded before running the benchmark.

\subsubsection{Image Classification}
Image classification is widely used in commercial applications and is also a de facto standard for evaluating ML-system performance. A classifier network takes an image as input and selects the class that best describes it. Example applications include photo searches, text extraction from images, and industrial automation, such as object sorting and defect detection.

For image classification, we use the standard ImageNet 2012 data set~\cite{deng2009imagenet} and crop to 224x224 during preprocessing. We selected two models: a higher-accuracy and more computationally expensive heavyweight model as well as a computationally lightweight model that is faster but less accurate.  Image-classification quality is the classifier's Top-1 accuracy.

The heavyweight model, ResNet-50 v1.5~\cite{he2016deep, mlperf2017resnet}, comes directly from the MLPerf Training suite to maintain alignment. ResNet-50 is the most common network for performance claims. Unfortunately, it has multiple subtly different implementations that make most comparisons difficult. In our training suite, we specifically selected ResNet-50 v1.5 to ensure useful comparisons and compatibility across major frameworks. We also extensively studied and characterized the network for reproducibility and low run-to-run training variation, making it an obvious and low-risk choice.

The lightweight model, MobileNets-v1 224~\cite{howard2017mobilenets}, is built around smaller, depth-wise-separable convolutions to reduce the model complexity and computational burden. MobileNets is a family of models that offer varying compute and accuracy options---we selected the full-width, full-resolution MobileNet-v1-1.0-224. This network reduces the parameters by 6.1x and the operations by 6.8x compared with ResNet-50 v1.5. We evaluated both MobileNet-v1 and v2~\cite{sandler2018mobilenetv2} for the MLPerf Inference v0.5 suite and selected the former, as it has garnered wider adoption.

\subsubsection{Object Detection}

Object detection is a complex vision task that determines the coordinates of bounding boxes around objects in an image and classifies the image. Object detectors typically use a pretrained image-classifier network as a backbone or a feature extractor, then perform regression for localization and bounding-box selection. Object detection is crucial for automotive applications, such as detecting hazards and analyzing traffic, and for mobile-retail tasks, such as identifying items in a picture. 

For object detection, we chose the COCO data set \cite{lin2014microsoft} with both a lightweight and heavyweight model. Our small model uses the 300x300 image size, which is typical of resolutions in smartphones and other compact devices. For the larger model, we upscale the data set to more closely represent the output of a high-definition image sensor (1.44~MP total). The choice of the larger input size is based on community feedback, especially from automotive and industrial-automation customers. The quality metric for object detection is mean average precision (mAP). 

The heavyweight object detector's reference model is SSD~\cite{liu2016ssd} with a ResNet34 backbone, which also comes from our training benchmark. The lightweight object detector's reference model uses a MobileNet-v1-1.0 backbone, which is more typical for constrained computing environments. We selected the MobileNet feature detector on the basis of feedback from the mobile and embedded communities.

\subsubsection{Translation}

Neural machine translation (NMT) is popular in the rapidly evolving field of natural-language processing. NMT models translate a sequence of words from a source language to a target language and are used in translation applications and services. Our translation data set is WMT16 EN-DE~\cite{wmt2016}. The quality measurement is Bilingual Evaluation Understudy Score (Bleu)~\cite{papineni2002bleu}. In MLPerf Inference, we specifically employ SacreBleu~\cite{post2018call}.

For the translation, we chose GNMT~\cite{wu2016google}, which employs a well-established recurrent-neural-network (RNN) architecture and is part of the training benchmark. GNMT is representative of RNNs, which are popular for sequential and time-series data, and it ensures our reference-model suite captures a wide variety of compute motifs.

\subsection{Quality Targets}
%Quality and performance are intimately connected for all forms of machine learning, but the role of quality targets in inference is distinct from training. For training, performance is measured by time-to-train to the quality metric, thus accuracy is a first-order consideration for performance. For inference, the starting point is a pre-trained reference model that achieves a target quality, but many system architectures are willing to trade model quality for lower latency or lower Total Cost of Ownership (TCO) via higher throughput. 
%
%The trade-offs between accuracy, latency, and TCO are application specific. Trading 1\% model accuracy for 50\% lower TCO seems prudent when identifying cat photos, but less prudent for online pedestrian detection. For the purposes of MLPerf, we need to define a model’s quality targets. 

Many architectures can trade model quality for lower latency, lower TCO, or greater throughput. To reflect this important aspect of real-world deployments, we established per-model and scenario targets for latency and model quality. We adopted quality targets that for 8-bit quantization were achievable with considerable effort.

MLPerf Inference requires that almost all implementations achieve a quality target within 1\% of the FP32 reference model's accuracy (e.g., the ResNet-50 v1.5 model achieves 76.46\% Top-1 accuracy, and an equivalent model must achieve at least 75.70\% Top-1 accuracy). Initial experiments, however, showed that for mobile-focused networks---MobileNet and SSD-MobileNet---the accuracy loss was unacceptable without retraining. We were unable to proceed with the low accuracy because performance benchmarking would become unrepresentative.

To address the accuracy drop, we took three steps. First, we trained the MobileNet models for quantization-friendly weights, enabling us to narrow the quality window to 2\%. Second, to reduce the training sensitivity of MobileNet-based submissions, we provided equivalent MobileNet and SSD-MobileNet implementations quantized to an 8-bit integer format. Third, for SSD-MobileNet, we reduced the quality requirement to 22.0~mAP to account for the challenges of using MobileNets as a backbone.

To improve the submission comparability, we disallow retraining. Our prior experience and feasibility studies confirmed that for 8-bit integer arithmetic, which was an expected deployment path for many systems, the $\sim$1\% relative-accuracy target was easily achievable without retraining. 

\subsection{Scenarios and Metrics}
\label{sec:benchmarks:scenarios}

% Another crucial difference between training and inference is the typical usage model and therefore the appropriate performance metrics. Training systems tend to range from powerful single systems to hundreds or even thousands of servers in a data center and each training session is long so that end-to-end latency is the best metric. 

%Inference systems vary across six or more orders of magnitude in power consumption and cover a wide variety of applications and physical deployments from deeply embedded devices to smartphones and data centers. 

The diverse inference applications have various usage models and figures of merit, which in turn require multiple performance metrics. To address these models, we specify four scenarios that represent important inference applications. Each one has a unique performance metric, as Table~\ref{tab:scenarios} illustrates. The LoadGen discussed in Section~\ref{sec:benchmarks:loadgen} simulates the scenarios and measures the performance.

%Inference systems vary across six or more orders of magnitude in power consumption and cover a wide variety of applications and physical deployments from deeply embedded devices to smartphones and data centers. The diverse set of inference applications have a variety of usage models and many different figures of merit, which in turn require multiple performance metrics. For example, the figure of merit for an image recognition system that is classifying the output of a video camera will be entirely different than for a cloud-based translation system.
%
%To address these different usage models, we surveyed the wide membership of MLPerf, which includes both customers and vendors. Based on the feedback, we specified four different scenarios that we believe represent many important inference applications. Each of the four scenarios has a unique performance metric, as illustrated in Table \ref{tab:scenarios}. The load generator (``LoadGen'') discussed in Section~\ref{sec:benchmarks:loadgen} simulates the scenarios and measures the performance.

\input{table/scenarios_description.tex}

\textbf{Single-stream.} This scenario represents one inference-query stream with a query sample size of one, reflecting the many client applications where responsiveness is critical. An example is offline voice transcription on Google's Pixel~4 smartphone. To measure performance, the LoadGen injects a single query; when the query is complete, it records the completion time and injects the next query. The performance metric is the query stream's 90th-percentile latency. 

\textbf{Multistream.} This scenario represents applications with a stream of queries, but each query comprises multiple inferences, reflecting a variety of industrial-automation and remote-sensing applications. For example, many autonomous vehicles analyze frames from six to eight cameras that stream simultaneously. 

To model a concurrent scenario, the LoadGen sends a new query comprising \emph{N} input samples at a fixed time interval (e.g., 50 ms). The interval is benchmark specific and also acts as a latency bound that ranges from 50 to 100 milliseconds. If the system is available, it processes the incoming query. If it is still processing the prior query in an interval, it skips the interval and delays the remaining queries by one interval. 

No more than 1\% of the queries may produce one or more skipped intervals. A query's \emph{N} input samples are contiguous in memory, which accurately reflects production input pipelines and avoids penalizing systems that would otherwise require that samples be copied to a contiguous memory region before starting inference. The performance metric is the integer number of streams that the system supports while meeting the QoS requirement.

\textbf{Server.} This scenario represents online server applications where query arrival is random and latency is important. Almost every consumer-facing website is a good example, including services such as online translation from Baidu, Google, and Microsoft. For this scenario, the load generator sends queries, with one sample each, in accordance with a Poisson distribution. The SUT responds to each query within a benchmark-specific latency bound that varies from 15 to 250 milliseconds. No more than 1\% of queries may exceed the latency bound for the vision tasks and no more than 3\% may do so for translation. The server scenario's performance metric is the Poisson parameter that indicates the queries per second achievable while meeting the QoS requirement.

\textbf{Offline.} This scenario represents batch-processing applications where all the input data is immediately available and latency is unconstrained. An example is identifying the people and locations in a photo album. For the offline scenario, the LoadGen sends  to the system a single query that includes all sample-data IDs to be processed, and the system is free to process the input data in any order. Similar to the multistream scenario, neighboring samples in the query are contiguous in memory. The metric for the offline scenario is throughput measured in samples per second.

For the multistream and server scenarios, latency is a critical component of the system behavior and will constrain various performance optimizations. For example, most inference systems require a minimum (and architecture-specific) batch size to achieve full utilization of the underlying computational resources. But in a server scenario, the arrival rate of inference queries is random, so systems must carefully optimize for tail latency and potentially process inferences with a suboptimal batch size. 

Table \ref{tab:latency} shows the relevant latency constraints for each task in v0.5. As with other aspects of MLPerf, we selected these constraints on the basis of community consultation and feasibility assessments. The multistream arrival times for most vision tasks correspond to a frame rate of 15--20 Hz, which is a minimum for many applications. The server QoS constraints derive from estimates of the inference timing budget given an overall user latency target.

\input{table/latency_constraints.tex}


\subsection{Statistical Confidence}
To ensure our results are statistically robust and adequately capture steady-state system behavior, each task and scenario combination requires a minimum number of queries. That number is determined by the tail-latency percentile, the desired margin, and the desired confidence interval. 

Confidence is the probability that a latency bound is within a particular margin of the reported result. We chose a 99\% confidence bound and set the margin to a value much less than the difference between the tail-latency percentage and 100\%. Conceptually, that margin ought to be relatively small. Thus, we selected a margin that is one-twentieth of the difference between the tail-latency percentage and 100\%. 

The equation is as follows:

\begin{small}
\begin{equation}
    Margin = \frac{1 - TailLatency}{20} 
\end{equation}  
\begin{equation}
\begin{aligned}
    {NumQueries} &= ({Normslnv}(\frac{1-{Confidence}}{2}))^{2}\\ &\times \frac{{TailLatency}\times({1 - TailLatency})}{{Margin}^2} 
\end{aligned}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     \text{NumQueries} &= (\text{Normslnv}(\frac{1-0.99}{2}))^{2} \times \frac{0.9 \times (1-0.9)}{0.005^2} \\
%     &= (\text{Normslnv}(0.005))^{2} \times 3600 \\
%     &= (-2.58)^{2} \times 3600 = 23886 
% \end{aligned}
% \end{equation}
\end{small}

Table \ref{tab:statsconf} shows the query requirements. The total query count and tail-latency percentile are scenario and task specific. The single-stream scenario only requires 1,024 queries, and the offline scenario requires a single query containing at least 24,576 samples. The single-stream scenario has the fewest queries to execute because we wanted the run time to be short enough that embedded platforms and smartphones could complete the runs quickly. 

\input{table/query_requirements.tex} 

For scenarios with latency constraints, our goal is to ensure a 99\% confidence interval that the constraints hold. As a result, the benchmarks with more-stringent latency constraints require more queries in a highly nonlinear fashion. The number of queries is based on the aforementioned statistics and is rounded up to the nearest multiple of $2^{13}$. 

A 99$^{th}$-percentile guarantee requires 262,742 queries, which rounds up to $33 \times 2^{13}$, or 270K. For both multistream and server, this guarantee for vision tasks requires 270K queries, as Table \ref{tab:task_queries} shows. Because a multistream benchmark will process $N$ samples per query, the total number of samples will be $N \times$ 270K. Machine translation has a 97$^{th}$-percentile latency guarantee and requires only 90K queries.

\input{table/model_queries.tex}

For repeatability, we run both the multistream and server scenarios several times. But the multistream scenario's arrival rate and query count  guarantee a 2.5- to 7-hour run time. To strike a balance between repeatability and run time, we require five runs for the server scenario, with the result being the minimum of these five runs. The other scenarios require one run. We expect to revisit this choice in future benchmark versions.

All benchmarks must also run for at least 60 seconds and process additional queries and/or samples as the scenarios require. The minimum run time ensures they will measure the equilibrium behavior of power-management systems and systems that support dynamic voltage and frequency scaling (DVFS), particularly for the single-stream scenario with a small number of queries.

\subsection{Load Generator}
\label{sec:benchmarks:loadgen}

The LoadGen is a traffic generator that loads the SUT and measures performance. Its behavior is controlled by a configuration file it reads at the start of the benchmark run. The LoadGen produces the query traffic according to the rules of the previously described scenarios (i.e., single-stream, multistream, server, and offline). Additionally, the LoadGen collects information for logging, debugging, and postprocessing the data. It records queries and responses from the SUT, and at the end of the run, it reports statistics, summarizes the results, and determines whether the run was valid.

Figure~\ref{fig:Loadgen} shows how the LoadGen generates query traffic for each scenario. In the server scenario, for instance, it issues queries in accordance with a Poisson distribution to mimic a server's query-arrival rates. In the single-stream case, it issues a query to the SUT and waits for completion of that query before issuing another. 


\subsubsection{Design}
MLPerf will evolve, introducing new tasks and removing old ones as the field progresses. Accordingly, the LoadGen's design is flexible enough to handle changes to the inference-task suite. We achieve this feat by decoupling the LoadGen from the benchmarks and the internal representations (e.g., the model,  scenarios, and quality and latency metrics). 

The LoadGen is implemented as a standalone C++ module with well-defined APIs; the benchmark calls it through these APIs (and vice versa through callbacks). This decoupling at the API level allows it to easily support various language bindings, permitting benchmark implementations in any language. Presently, the LoadGen supports Python, C, and C++ bindings; additional bindings can be added.

Another major benefit of decoupling the LoadGen from the benchmark is that the LoadGen is extensible to support more scenarios. Currently,  MLPerf supports four of them; we may add more, such as a multitenancy mode where the SUT must continuously serve multiple models while maintaining QoS constraints.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/LoadGen_Scenarios.pdf}
    \caption{The timing and number of queries from the Load Generator (LoadGen) vary between benchmark scenarios. All five ML tasks can run in any one of the four scenarios.}
    \label{fig:Loadgen}
    \vskip -0.15in
\end{figure}


\subsubsection{Implementation}
The LoadGen abstracts the details of the data set (e.g., images) behind sample IDs. Data-set samples receive an index between 0 and \emph{N}. A query represents the smallest input unit that the benchmark ingests from the LoadGen. It consists of one or more data-set sample IDs, each with a corresponding response ID to differentiate between multiple instances of the same sample. 

The rationale for a response ID is that for any given task and scenario---say, an image-classification multistream scenario---the LoadGen may reissue the same data (i.e., an image with a unique sample ID) multiple times across the different streams. To differentiate between them, the LoadGen must assign different reference IDs to accurately track when each sample finished processing.

At the start, the LoadGen directs the benchmark to load a list of samples into memory. Loading is untimed and the SUT may also perform allowed data preprocessing. The LoadGen then issues queries, passing sample IDs to the benchmark for execution on the inference hardware. The queries are pre-generated to reduce overhead during the timed portion of the test.

As the benchmark finishes processing the queries, it informs the LoadGen through a function named \textit{QuerySamplesComplete}. The LoadGen makes no assumptions regarding how the SUT may partition its work, so any thread can call this function with any set of samples in any order. \textit{QuerySamplesComplete} is thread safe, is wait-free bounded, and makes no syscalls, allowing it to scale recording to millions of samples per second and to minimize the performance variance introduced by the LoadGen, which would affect long-tail latency.

The LoadGen maintains a logging thread that gathers events as they stream in from other threads. At the end of the benchmark run, it outputs a set of logs that report the performance and accuracy stats.

\subsubsection{Operating Modes}
The LoadGen has two primary operating modes: {accuracy} and {performance}. Both are necessary to make a valid MLPerf submission.

{\bf Accuracy mode.} The LoadGen goes through the entire data set for the ML task. The model's task is to run inference on the complete data set. Afterward, accuracy results appear in the log files, ensuring that the model met the required quality target.

{\bf Performance mode.} The LoadGen avoids going through the entire data set, as the system's performance can be determined by subjecting it to enough data-set samples. 

% So the LoadGen generates traffic until the benchmark has processed the minimum number of queries required for the specific task and scenario combination, and the benchmark has executed for at least 60 seconds. At the end of the run, the LoadGen outputs log files with query processing latency percentiles and other statistics for post-processing the system’s performance.

%\subsubsection{Features}
%
%There are several validation features supported by the LoadGen to help detect SUT behavior not allowed by the rules. These features can be controlled by an audit.config file that the LoadGen searches for in the working directory. The audit.config file overrides all other settings requested by the SUT. See Section~\ref{sec:submission} for review and validation details.

\subsubsection{Validation Features}\label{sec:benchmarks:loadgen_validation}

The LoadGen has features that ensure the submission system complies with the rules. In addition, it can self-check to determine whether its source code has been modified during the submission process. To facilitate validation, the submitter provides an experimental config file that allows use of non-default LoadGen features. For v0.5, the LoadGen enables the following three tests.

\textbf{Accuracy verification.}
The purpose of this test is to ensure valid inferences in performance mode. By default, the results that the inference system returns to the LoadGen are not logged and thus are not checked for accuracy. This choice reduces or eliminates processing overhead to allow accurate measurement of the inference system's performance. In this test, results returned from the SUT to the LoadGen are logged randomly. The log is checked against the log generated in accuracy mode to ensure consistency.

\textbf{On-the-fly caching detection.}
By default, LoadGen produces queries by randomly selecting with replacement from the data set, and inference systems may receive queries with duplicate samples. This outcome is likely for high-performance systems that process many samples relative to the data-set size. To represent realistic deployments, the MLPerf rules prohibit caching of queries or intermediate data. The test has two parts. The first part generates queries with unique sample indices. The second generates queries with duplicate sample indices. Performance is measured in each case. The way to detect caching is to determine whether the test with duplicate sample indices runs significantly faster than the test with unique sample indices.

\textbf{Alternate-random-seed testing.}
In ordinary operation, the LoadGen produces queries on the basis of a fixed random seed. Optimizations based on that seed are prohibited. The alternate-random-seed test replaces the official random seed with alternates and measures the resulting performance.

%\subsubsection{Custom datasets}
%Inference systems are prohibited from precalculating results. This behavior is validated by replacing the reference data set with a different custom data set. The quality and performance of the system operating on the custom data set are measured and compared against operation with the reference data set.

\subsection{Model Equivalence}

The goal of MLPerf Inference is to measure realistic system-level performance across a wide variety of architectures. But the four properties of realism, comparability, architecture neutrality, and friendliness to small submission teams require careful trade-offs. 

Some inference deployments involve teams of compiler, computer-architecture, and machine-learning experts aggressively co-optimizing the training and inference systems to achieve cost, accuracy, and latency targets across a massive global customer base. An unconstrained inference benchmark, however, would disadvantage companies with less experience and fewer ML-training resources.

Therefore, we set the model-equivalence rules to allow submitters to, for efficiency, reimplement models on different architectures. The rules provide a complete list of disallowed techniques and a list of allowed technique examples. We chose an explicit blacklist to encourage a wide range of techniques and to support architectural diversity. The list of examples illustrates the boundaries of the blacklist while also encouraging common and appropriate optimizations. 

Examples of allowed techniques include the following: arbitrary data arrangement as well as different input and in-memory representations of weights, mathematically equivalent transformations (e.g., tanh versus logistic, ReluX versus ReluY, and any linear transformation of an activation function), approximations (e.g., replacing a transcendental function with a polynomial), processing queries out of order within the scenario's limits, replacing dense operations with mathematically equivalent sparse operations, fusing or unfusing operations, dynamically switching between one or more batch sizes, mixing experts that combine differently quantized weights. 

% Examples of disallowed techniques include, but are not limited to: wholesale weight replacement or supplements; discarding non-zero weight elements, including pruning; caching queries or responses; coalescing identical queries; techniques that boost performance for fixed length experiments but are inapplicable to long-running services except in the offline scenario; techniques that only improve performance when there are identical samples.

\subsubsection{Prohibited Optimizations}
MLPerf Inference currently prohibits retraining and pruning to ensure comparability, although this restriction may fail to reflect realistic deployment for some large companies. The interlocking requirements to use reference weights (possibly with calibration) and minimum accuracy targets are most important for ensuring comparability in the closed division. The open division explicitly allows retraining and pruning.

We prohibit caching to simplify the benchmark design. In practice, real inference systems cache queries. For example, \emph{``I love you''} is one of Google Translate's most frequent queries, but the service does not translate the phrase \textit{ab initio} each time. Realistically modeling caching in a benchmark, however, is a challenge because cache hit rates vary substantially with the application. Furthermore, our data sets are relatively small, and large systems could easily cache them in their entirety. 

We also prohibit optimizations that are benchmark aware or data-set aware and that are inapplicable to production environments. For example, real query traffic is unpredictable, but for the benchmark, the traffic pattern is predetermined by the pseudorandom-number-generator seed. Optimizations that take advantage of a fixed number of queries or that use knowledge of the LoadGen implementation are prohibited. Similarly, any optimization employing statistical knowledge of the performance or accuracy data sets is prohibited. Finally, we disallow any technique that takes advantage of the upscaled images in the 1,200x1,200 COCO data set for the heavyweight object detector.

\subsubsection{Preprocessing and Data Types}
Ideally, a whole-system benchmark should capture all performance-relevant operations. MLPerf, however, explicitly allows untimed preprocessing. There is no vendor- or application-neutral preprocessing. For example, systems with integrated cameras can use hardware/software co-design to ensure that images arrive in memory in an ideal format; systems accepting JPEGs from the Internet cannot.

In the interest of architecture and application neutrality, we adopted a permissive approach to untimed preprocessing. Implementations may transform their inputs into system-specific ideal forms as an untimed operation.

MLPerf explicitly allows and enables quantization to a wide variety of numerical formats to ensure architecture neutrality. Submitters must pre-register their numerics to help guide accuracy-target discussions. The approved list for the closed division includes INT4, INT8, INT16, UINT8, UINT16, FP11 (sign, 5-bit mantissa, and 5-bit exponent), FP16, bfloat16, and FP32. 

Quantization to lower-precision formats typically requires calibration to ensure sufficient inference quality. For each reference model, MLPerf provides a small, fixed data set that can be used to calibrate a quantized network. Additionally, it offers MobileNet versions that are prequantized to INT8, since without retraining (which we disallow) the accuracy falls dramatically.

==> tex/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

More than 200 ML researchers, practitioners, and engineers from academia and industry helped to bring the MLPerf Inference benchmark from concept (June 2018) to result submission (October 2019). This team, drawn from 32 organizations, developed the reference implementations and rules, and submitted over 600 performance measurements gathered on a wide range of systems. Of these performance measurements, 595 cleared the audit process as valid submissions and were approved for public consumption.  

MLPerf Inference v0.5 is just the beginning. The key to any benchmark's success, especially in a rapidly changing field such as ML, is a development process that can respond quickly to changes in the ecosystem. Work has already started on the next version. We expect to update the current models (e.g., MobileNet-v1 to v2), expand the list of tasks (e.g., recommendation), increase the processing requirements by scaling the data-set sizes (e.g., 2 MP for SSD large), allow aggressive performance optimizations (e.g., retraining for quantization), simplify benchmarking through better infrastructure (e.g., a mobile app), and increase the challenge to systems by improving the metrics (e.g., measuring power and adjusting the quality targets).

We welcome your input and contributions. Visit the MLPerf website (\url{https://mlperf.org}) for additional details. Results for v0.5 are available online (\url{https://github.com/mlperf/inference_results_v0.5}).


==> tex/goals.tex <==
\section{MLPerf Inference Goals}
\label{sec:goals}

To overcome the challenges, MLPerf Inference adopted a set of principles for developing a robust yet flexible benchmark suite based on community-driven development.

\subsection{Representative, Broadly Accessible Workloads} 

For the initial version 0.5, we chose tasks that reflect major commercial and research scenarios for a large class of submitters and that capture a broad set of computing motifs. To focus on the realistic rules and testing infrastructure, we selected a minimum-viable-benchmark approach to accelerate the development process. Where possible, we adopted models that were part of the MLPerf Training v0.6 suite~\cite{mattson2019mlperf}, thereby amortizing the benchmark-development effort. 

The current version's tasks and models are modest in scope. MLPerf Inference v0.5 comprises three tasks and five models: image classification (ResNet-50~\cite{he2016deep} and MobileNet-v1~\cite{howard2017mobilenets}), object detection (SSD-ResNet34\textemdash i.e., SSD~\cite{liu2016ssd} with a ResNet34 backbone\textemdash and SSD-MobileNet-v1\textemdash i.e., SSD with a MobileNet-v1 backbone), and machine translation (GNMT~\cite{wu2016google}). We plan to add others.

We chose our tasks and models through a consensus-driven process and considered community feedback to ensure their relevance. Our models are mature and have earned broad community support. Because the industry has studied them and can build efficient systems, benchmarking is accessible and provides a snapshot that shows the state of ML systems. Moreover, we focused heavily on the benchmark's modular design to make adding new models and tasks less costly. As we show in Section~\ref{sec:results_open_division}, our design has allowed MLPerf Inference users to easily add new models. Our plan is to extend the scope to include more areas, tasks, models, and so on. Additionally, we aim to maintain consistency and alignment between the training and inference benchmarks.

\subsection{System Evaluation Using Realistic Scenarios}

As our submission results show, ML inference systems vary in power consumption across four or more orders of magnitude and cover a wide variety of applications as well as physical deployments that range from deeply embedded devices to smartphones to data centers. The applications have a variety of usage models and many figures of merit, which in turn require multiple performance metrics. For example, the figure of merit for an image-recognition system that classifies a video camera's output will be entirely different than for a cloud-based translation system. To address these various models, we surveyed MLPerf's broad membership, which includes both customers and vendors. On the basis of that feedback, we identified four scenarios that represent many critical inference applications. 

Our goal is a method that simulates the realistic behavior of the inference system under test; such a feature is unique among AI benchmarks. To this end, we developed the Load Generator (LoadGen) tool, which is a query-traffic generator that mimics the behavior of real-world systems. It has four scenarios: \emph{single-stream}, \emph{multistream}, \emph{server} and \emph{offline}. They emulate the ML-workload behavior of mobile devices, autonomous vehicles, robotics, and cloud-based setups. 

% The LoadGen builds upon principles borrowed from networking and distributed systems about query arrival rates, queuing, etc.~\cite{}. [https://ai.google/research/pubs/pub40801, http://cseweb.ucsd.edu/~gmporter/classes/fa17/cse124/post/schedule/p74-dean.pdf].

\subsection{Target Qualities and Tail-Latency Bounds} 

Quality and performance are intimately connected for all forms of machine learning, but the role of quality targets in inference is distinct from that in training. For training, the performance metric is the time to train to a specific quality, making accuracy a first-order consideration. For inference, the starting point is a pretrained reference model that achieves a target quality. Still, many system architectures can sacrifice model quality to achieve lower latency, lower total cost of ownership (TCO), or higher throughput.

The trade-offs between accuracy, latency, and TCO are application specific. Trading 1\% model accuracy for 50\% lower TCO is prudent when identifying cat photos, but it is less so during online pedestrian detection. For MLPerf, we define a model's quality targets. To reflect this important aspect of real world-deployments, we established per-model and scenario targets for inference latency and model quality. The latency bounds and target qualities are based on input gathered from end users. 

\subsection{Flexibility to Showcase Hardware and Software} 

Systems benchmarks can be characterized as language level (SPECInt~\cite{dixit1991spec}), API level (LINPACK~\cite{Dongarra1988linpack}), or semantic level (TPC~\cite{council2005transaction}). The ML community has embraced a wide variety of languages and libraries, so MLPerf Inference is a semantic-level benchmark. This type specifies the task to be accomplished and the general rules of the road, but it leaves implementation details to the submitters. 

The MLPerf Inference benchmarks are flexible enough that submitters can optimize the reference models, run them through their preferred software tool chain, and execute them on their hardware of choice. Thus, MLPerf Inference has two divisions: closed and open. Strict rules govern the closed division, whereas the open division is more permissive and allows submitters to change the model, achieve different quality targets, and so on. The closed division is designed to address the lack of a standard inference-benchmarking workflow. 

Within each division, submitters may file their results under specific categories on the basis of their hardware and software components' availability. There are three system categories: available; preview; and research, development, or other systems. Systems in the first category are available off the shelf, while systems in the second category allow vendors to provide a sneak peek into their capabilities. At the other extreme are bleeding-edge ML solutions in the third category that are not ready for production use.

In summary, MLPerf Inference allows submitters to exhibit many different systems across varying product-innovation, maturity, and support levels.

\subsection{Benchmark Changes for Rapidly Evolving ML} 
MLPerf Inference v0.5 is only the beginning. The benchmark will evolve. We are working to add more models (e.g., recommendation and time-series models), more scenarios (e.g., ``burst'' mode), better tools (e.g., a mobile application), and better metrics (e.g., timing preprocessing) to more accurately reflect the performance of the whole ML pipeline. 

==> tex/lessons.tex <==
\section{Lessons Learned}
\label{sec:lessons}

We reflect on our v0.5 benchmark-development effort and share some lessons we learned from the experience. 

\subsection{Community-Driven Benchmark Development}
\label{sec:community}

There are two main approaches to building an industry-standard benchmark. One is to create the benchmark in house, release it, and encourage the community to adopt it. The other is first to consult the community and then build the benchmark through a consensus-based effort. The former approach is useful when seeding an idea, but the latter is necessary to develop an industry-standard benchmark. MLPerf Inference employed the latter. 

MLPerf Inference began as a community-driven effort on July 12, 2018. We consulted more than 15 organizations. Since then, many other organizations have joined the MLPerf Inference working group. Applying the wisdom of several ML engineers and practitioners, we built the benchmark from the ground up, soliciting input from the ML-systems community as well as hardware end users. This collaborative effort led us to directly address the industry's diverse needs from the start. For instance, the LoadGen and scenarios emerged from our desire to span the many inference-benchmark needs of various organizations.

Although convincing competing organizations to agree on a benchmark is a challenge, it is still possible---as MLPerf Inference shows. Every organization has unique requirements and expectations, so reaching a consensus was sometimes tricky. In the interest of progress, everyone agreed to make decisions on the basis of ``grudging consensus.'' These decisions were not always in favor of any one organization. Organizations would comply to keep the process moving or defer their requirements to a future version so benchmark development could continue.

Ultimately, MLPerf Inference exists because competing organizations saw beyond their self-interest and worked together to achieve a common goal: establishing the best ways to measure ML inference performance.

\subsection{Perfect Is the Enemy of Good}

MLPerf Inference v0.5 has a modest number of tasks and models. Early in the development process, it was slated to cover 11 ML tasks: image classification, object detection, speech recognition, machine translation, recommendation, text (e.g., sentiment) classification, language modeling, text to speech, face identification, image segmentation, and image enhancement. We chose these tasks to cover the full breadth of ML applications relevant to the industry. 

As it matured, however, engineering hurdles and the participating organizations' benchmark-carrying capacity limited our effort. The engineering hurdles included specifying and developing the LoadGen system, defining the scenarios, and building the reference implementations. The LoadGen, for instance, involved 11 engineers from nine organizations. The reference implementations involved 34 people from 15 organizations contributing to our GitHub repository. 

We deemed that overcoming the engineering hurdles was a priority, as they would otherwise limit our ability to represent various workloads and to grow in the long term. Hence, rather than incorporating many tasks and models right away, we trimmed the number of tasks to five and focused on developing a proper method and infrastructure. 

With the hurdles out of the way, a small team or even an individual can add new models. For instance, thanks to the LoadGen and a complementary workflow-automation technology~\cite{fursin2016collective}, one MLPerf contributor with only three employees swept more than 60 computer-vision models in the open division.

Similarly, adding another task would require only a modest effort to integrate with the LoadGen and implement the model. This flexibility allows us to accommodate the changing ML landscape, and it saves practitioners and researchers from having to perform these explorations manually, all while showcasing potential techniques and optimizations for future versions of the closed division. 

\subsection{Audits and Auditability}

MLPerf is committed to integrity through rigorous submitter cross-auditing and to the privacy of the auditing process. This process was uncontentious and smooth flowing. Three innovations helped ease the audit process: permissive rules, the LoadGen, and the submission checker. 

% The complexity of enforcement and adjudication increases with the number of rules; consider tax law, for instance. Prior MLPerf Training rounds white-listed specific techniques, but an explicit white list produced an effectively infinite blacklist and paved the way for rule disputes. By contrast, a small explicit blacklist is easier to understand, interpret, and enforce. 

Concerns arose during rule-making that submitters would discover loopholes in the blacklist, allowing them to ``break'' the benchmark and, consequently, undermine the legitimacy of the entire MLPerf project. Submitters worked together to patch loopholes as they appeared because all are invested in the success of the benchmark.

The LoadGen improved auditability by separating measurement and experimental setup into a shared component. The only possible error in the experimental procedure is use of the wrong LoadGen settings. The LoadGen, therefore, significantly reduced compliance issues.

Finally, MLPerf provided a script for checking submissions. The script allowed submitters to verify that they submitted all required files in the right formats along with the correct directory layouts. It also verified LoadGen settings and scanned logs for noncompliance. 

The submission-checker script kept all submissions relatively uniform and allowed submitters to quickly identify and resolve potential problems. In future revisions, MLPerf will aim to expand the range of issues the submission script discovers. We also plan to include additional checker scripts and tools to further smooth the audit process.

% \subsection{Accuracy and Usability}

% The three most important aspects for evaluating an inference system are performance, accuracy, and usability. Currently, MLPerf only addresses the first of these aspects. Ideally, future rounds will improve on this foundation. 

% MLPerf Inference 0.5 set accuracy targets at 32-bit floating point accuracy minus one percent in order to facilitate eight-bit quantized submissions without retraining. Consequently, almost all results feature eight-bit quantization even when hardware supports more precise numerics. It is easy to read the results table as saying, ``The future is eight-bit,'' but this result actually reflects MLPerf's choice of target accuracy. One percent accuracy loss is fine for some applications, but too much for others. Could eight-bit quantization hit higher accuracy targets with retraining? Future rounds of MLPerf ought to more fully characterize the space of performance accuracy tradeoffs. Futhermore, retraining improves the accuracy of quantization. MLPerf ought to develop rules permitting retraining.

% Datacenter inferences are astonishingly cheap, and ML developers are staggeringly expensive. An enormous number of worked for more than three months to achieve performance results (Section~\ref{sec:acks}). Are these results representative for organizations with smaller teams of developers and less ML expertise? Future revisions of MLPerf ought to reflect both out-of-the-box performance and expert tuned performance.

==> tex/related.tex <==
\section{Prior Art in AI/ML Benchmarking}
\label{sec:priorart}

The following summary describes prior AI/ML inference benchmarking. Each of these benchmarks has made unique contributions. MLPerf has strived to incorporate and build on the best aspects of previous work while ensuring it includes community input. Compared with earlier efforts, MLPerf brings more-rigorous performance metrics that we carefully selected for each major use case along with a much wider (but still compact) set of ML applications and models based on the community's input.

\textbf{AI Benchmark.} AI Benchmark~\cite{ignatov2019ai} is arguably the first mobile-inference benchmark suite. It covers 21 computer-vision and AI tests grouped in 11 sections. These tests are predominantly computer-vision tasks (image recognition, face detection, and object detection), which are also well represented in the MLPerf suite. The AI Benchmark results and leaderboard focus primarily on Android smartphones and only measure inference latency. The suite provides a summary score, but it does not explicitly specify the quality targets. Relative to AI Benchmark, we aim at a wider variety of devices (submissions for v0.5 range from IoT devices to server-scale systems) and multiple scenarios. Another important distinction is that MLPerf does not endorse a summary score, as we mentioned previously.

\textbf{EEMBC MLMark.} EEMBC MLMark~\cite{eembc} is an ML benchmark suite designed to measure the performance and accuracy of embedded inference devices. It includes image-classification (ResNet-50 v1 and MobileNet-v1) and object-detection (SSD-MobileNet-v1) workloads, and its metrics are latency and throughput. Its latency and throughput modes are roughly analogous to the MLPerf single-stream and offline modes. MLMark measures performance at explicit batch sizes, whereas MLPerf allows submitters to choose the best batch sizes for different scenarios. Also, the former imposes no target-quality restrictions, whereas the latter imposes stringent restrictions.

\textbf{Fathom.} An early ML benchmark, Fathom~\cite{adolf2016fathom} provides a suite of neural-network models that incorporate several types of layers (e.g., convolution, fully connected, and RNN). Still, it focuses on throughput rather than accuracy. Fathom was an inspiration for MLPerf: in particular, we likewise included a suite of models that comprise various layer types. Compared with Fathom, MLPerf provides both PyTorch and TensorFlow reference implementations for optimization, ensuring that the models in both frameworks are equivalent, and it also introduces a variety of inference scenarios with different performance metrics.

\textbf{AIXPRT.} Developed by Principled Technologies, AIXPRT~\cite{aixprt} is a closed, proprietary AI benchmark that emphasizes ease of use. It consists of image-classification, object-detection, and recommender workloads. AIXPRT publishes prebuilt binaries that employ specific inference frameworks on supported platforms. The goal of this approach is apparently to allow technical press and enthusiasts to quickly run the benchmark. Binaries are built using Intel OpenVino, TensorFlow, and NVIDIA TensorRT tool kits for the vision workloads, as well as MXNet for the recommendation system. AIXPRT runs these workloads using FP32 and INT8 numbers with optional batching and multi-instance, and it evaluates performance by measuring latency and throughput. The documentation and quality requirements are unpublished but are available to members. In contrast, MLPerf tasks are supported on any framework, tool kit, or OS; they have precise quality requirements; and they work with a variety of scenarios.

\textbf{AI Matrix.} AI Matrix~\cite{aimatrix} is Alibaba's AI-accelerator benchmark for both cloud and edge deployment. It takes the novel approach of offering four benchmark types. First, it includes micro-benchmarks that cover basic operators such as matrix multiplication and convolutions that come primarily from DeepBench. Second, it measures performance for common layers, such as fully connected layers. Third, it includes numerous full models that closely track internal applications. Fourth, it offers a synthetic benchmark designed to match the characteristics of real workloads. The full AI Matrix models primarily target TensorFlow and Caffe, which Alibaba employs extensively and which are mostly open source. 
We have a smaller model collection and focus on simulating scenarios using LoadGen.

\textbf{DeepBench.} Microbenchmarks such as DeepBench~\cite{baidu2017deepbench} measure the library implementation of kernel-level operations (e.g., 5,124x700x2,048 GEMM) that are important for performance in production models. They are useful for efficient model development but fail to address the complexity of testing and evaluating full ML models.

\textbf{TBD (Training Benchmarks for DNNs).} TBD~\cite{zhu2018tbd} is a joint project of the University of Toronto and Microsoft Research that focuses on ML training. It provides a wide spectrum of ML models in three frameworks (TensorFlow, MXNet, and CNTK), along with a powerful tool chain for their improvement. It primarily focuses on evaluating GPU performance and only has one full model (Deep Speech 2) that covers inference. We considered including TBD's Deep Speech 2 model but lacked the time.

\textbf{DAWNBench.} DAWNBench~\cite{coleman2017dawnbench} was the first multi-entrant benchmark competition to measure the end-to-end performance of deep-learning systems. It allowed optimizations across model architectures, optimization procedures, software frameworks, and hardware platforms. DAWNBench inspired MLPerf, but our benchmark offers more tasks, models, and scenarios.

To summarize, MLPerf Inference builds on the best of prior work and improves on it, in part through community-driven feedback (Section~\ref{sec:community}). The result has been new features, such as the LoadGen (which can run models in different scenarios), the open and closed divisions, and so on.


==> tex/results.tex <==
\section{Results}
\label{sec:results}

We received over 600 submissions in all three categories (available, preview, and RDO) across the closed and open divisions. Our results are the most extensive corpus of inference performance data available to the public, covering a range of ML tasks and scenarios, hardware architectures, and software run times. Each has gone through extensive review before receiving approval as a valid MLPerf result. After review, we cleared 595 results as valid. 

We evaluated the closed-division results on the basis of four of the five objectives our benchmark aimed to achieve. The exception is setting target qualities and tail-latency bounds in accordance with real use cases, which we do not discuss because a static benchmark setting applies to every inference task. Omitting that isolated objective, we present our analysis as follows:

\begin{itemize}
\setlength\itemsep{0em}

    \item Pick representative workloads that everyone can access (Sections~\ref{sec:results_accessibility} and~\ref{sec:results_task_coverage}).

    \item Evaluate systems in realistic scenarios (Section~\ref{sec:results_scenarios}).
    
    \item Allow the benchmark to flexibly showcase both hardware and software capabilities (Sections~\ref{sec:results_diversity_arch}, \ref{sec:results_diversity_sw},  and \ref{sec:results_diversity_systems}).
   
    \item Permit the benchmark to change rapidly in response to the evolving ML ecosystem (Section~\ref{sec:results_open_division}).
\end{itemize}

\setlength{\fboxsep}{0pt}
\begin{figure}[t!]
    \centering
    \vspace*{5pt}
    \fbox{\includegraphics[width=0.99\linewidth]{figures/map.png}}
    \caption{MLPerf Inference's accessibility and global reach. The organizations responding to the v0.5 call for submissions hail from around the world, including the United States, Canada, the European Union, Russia, the Middle East, India, China, and South Korea. This domestic and international adoption reflects the community's perspective that the benchmark is comprehensive and scientifically rigorous, and worthy of engineering time for submissions.}
    \label{fig:map}
    \vskip -0.15in
\end{figure}

\subsection{Accessibility and Global Reach}
\label{sec:results_accessibility}
A primary goal for MLPerf Inference was to create a widely available benchmark. To this end, the first round of submissions came from 14 worldwide organizations, hailing from the United States, Canada, Russia, the European Union, the Middle East, India, China, and South Korea, as Figure~\ref{fig:map} shows.

The submitters represent many organizations that range from startups to original equipment manufacturers (OEMs), cloud-service providers, and system integrators. They include Alibaba, 
Centaur Technology, Dell EMC, dividiti, FuriosaAI, Google, Habana, Hailo, Inspur, Intel, NVIDIA, Polytechnic University of Milan, Qualcomm, and Tencent.


\subsection{Task Coverage}
\label{sec:results_task_coverage}

MLPerf Inference v0.5 submitters are allowed to pick any task to evaluate their system's performance. The distribution of results across tasks can thus reveal whether those tasks are of interest to ML-system vendors. 

We analyzed the submissions to determine the overall task coverage. Figure~\ref{fig:closed_division} shows the breakdown for the tasks and models in the closed division. Although the most popular model was, unsurprisingly, ResNet-50 v1.5, it was just under three times as popular as GNMT, the least popular model. This small spread and the otherwise uniform distribution suggests we selected a representative set of tasks.

In addition to selecting representative tasks, another goal is to provide vendors with varying quality and performance targets. Depending on the use case, the ideal ML model may differ (as Figure~\ref{fig:ml_model} shows, a vast range of models can target a given task). Our results reveal that vendors equally supported different models for the same task because each model has unique quality and performance trade-offs. In the case of object detection, we saw the same number of submissions for both SSD-MobileNet-v1 and SSD-ResNet34.

% We see slightly more interest in image classification (MobileNets-v1 and ResNet-50 v1.5) than object detection, however.

\begin{figure}[t]
    \centering
    \vspace*{2pt}
    \fbox{\includegraphics[width=\columnwidth]{figures/piechart.pdf}}
    \caption{Results from the closed division. The distribution of models indicates MLPerf Inference capably selected representative workloads for the initial v0.5 benchmark release.}
    \label{fig:closed_division}
    \vskip -0.15in
\end{figure}

\subsection{Scenario Usage}
\label{sec:results_scenarios}

We aim to evaluate systems in realistic use cases---a major motivator for the LoadGen (Section \ref{sec:benchmarks:loadgen}) and scenarios (see Section \ref{sec:benchmarks:scenarios}). To this end, Table~\ref{tab:submissions} shows the distribution of results across the various task and scenario combinations. 

Across all the tasks, the single-stream and offline scenarios are the most widely used and are also the easiest to optimize and run. Server and multistream were more complicated and had longer run times because of the QoS requirements and more-numerous queries. 

GNMT garnered no multistream submissions, possibly because the constant arrival interval is unrealistic in machine translation. Therefore, it was the only model and scenario combination with no submissions.
\input{table/submissions.tex}

\subsection{Processor Types}
\label{sec:results_diversity_arch}
Machine-learning solutions can be deployed on a variety of platforms, ranging from fully general-purpose CPUs to programmable GPUs and DSPs, FPGAs, and fixed-function accelerators. Our results reflect this diversity. 

Figure~\ref{fig:submitted} shows that the MLPerf Inference submissions covered most hardware categories. The system diversity indicates that our inference benchmark suite and method for v0.5 can evaluate any processor architecture.

\begin{figure}[t]
    \centering
    \vspace*{4pt}
    \fbox{\includegraphics[width=\columnwidth]{figures/stacked.pdf}}
    \caption{Results from the closed division. The results cover many processor architectures. Almost every kind---CPUs, GPUs, DSPs, FPGAs, and ASICs---appeared in the submissions.}
    \label{fig:submitted}
    \vskip -0.15in
\end{figure}

\subsection{Software Frameworks}
\label{sec:results_diversity_sw}

In addition to the various hardware types are many ML software frameworks. Table \ref{tab:frameworks} shows the variety of frameworks used to benchmark the hardware platforms. ML software plays a vital role in unleashing the hardware's performance. 

Some run times are specifically designed to work with certain types of hardware to fully harness their capabilities; employing the hardware without the corresponding framework may still succeed, but the performance may fall short of the hardware's potential. The table shows that CPUs have the most framework diversity and that TensorFlow has the most architectural variety.

\subsection{Diversity of Systems}
\label{sec:results_diversity_systems}

The MLPerf Inference v0.5 submissions cover a broad range of systems on the power and performance scale, from mobile and edge devices to cloud computing. The performance delta between the smallest and largest inference systems is four orders of magnitude, or about 10,000x.

Table~\ref{tab:performance} shows the performance range for each task and scenario in the closed division (except for GNMT, which had no multistream submissions). For example, in the case of ResNet-50 v1.5 offline, the highest-performing system is over 10,000x faster than the lowest-performing one. Unsurprisingly, the former comprised multiple ML accelerators, whereas the latter was a low-power laptop-class CPU. This delta for single-stream is surprising given that additional accelerators cannot reduce latency, and it reflects an even more extensive range of systems than the other scenarios. In particular, the single-stream scenario includes many smartphone processors, which target very low power.

\input{table/frameworks.tex}

\input{table/performance_summary.tex}

Figure~\ref{fig:violin} shows the results across all tasks and scenarios. In cases such as the MobileNet-v1 single-stream scenario (SS), ResNet-50 v1.5 SS, and SSD-MobileNet-v1 SS, systems exhibit a large performance difference (100x). Because these models have many applications, the systems that target them cover everything from low-power embedded devices to high-performance servers. GNMT server (S) shows much less performance variation between systems.

\begin{figure*}[t!]
    \centering
    \vspace*{5pt}
    \includegraphics[width=\columnwidth]{figures/violin.pdf}
    \caption{Results from the closed division. Normalized performance distribution on log scale (log$_{10}$) across models for the single-stream~(SS), multistream~(MS), server~(S), and offline~(O) scenarios. The boxplot shows the performance distribution of all system submissions for a specific model and scenario combination. The results are normalized to the slowest system representing that combination. A wide range emerges across all tasks and scenarios. GNMT MS is absent because no submitter ran the multistream scenario.}
    \label{fig:violin}
    \vskip -0.15in 
\end{figure*}

The broad performance range implies that the selected tasks (as a starting point) for MLPerf Inference v0.5 are general enough to represent a variety of use cases and market segments. The wide array of systems also indicates that our method (LoadGen, metrics, etc.) is broadly applicable.


\subsection{Open Division}
\label{sec:results_open_division}
The open division is the vanguard of MLPerf's benchmarking efforts. It is less rigid than the closed division; we received over 400 results. The submitters ranged from startups to large organizations. 

A few highlights from the open division are the use of 4-bit quantization to boost performance, an exploration of a wide range of models to perform the ML task (instead of using the reference model), and a demonstration of one system's ability to deliver high throughput even under tighter latency bounds---tighter than those in the closed-division rules. 

In addition, we received a submission that pushed the limits of mobile-chipset performance. Typically, most vendors use one accelerator at a time to do inference. In this case, a vendor concurrently employed multiple accelerators to deliver high throughput in a multistream scenario---a rarity in conventional mobile use cases. Nevertheless, it shows that the MLPerf Inference open division is encouraging the industry to push the limits of systems.

In yet another interesting submission, two organizations jointly evaluated 12 object-detection models---YOLO v3~\cite{redmon2018yolov3}, Faster-RCNN~\cite{ren2015faster} with a variety of backbones, and SSD~\cite{liu2016ssd}) with a variety of backbones---on a desktop platform.
The open-division results save practitioners and researchers from having to manually perform similar explorations, while also showcasing potential techniques and optimizations.

